Misinformation Resilient Search Rankings with Webgraph-based Interventions

The proliferation of unreliable news domains on the internet has had wide-reaching negative impacts on society. We introduce and evaluate interventions aimed at reducing traffic to unreliable news domains from search engines while maintaining traffic to reliable domains. We build these interventions on the principles of fairness (penalize sites for what is in their control), generality (label/fact-check agnostic), targeted (increase the cost of adversarial behavior), and scalability (works at webscale). We refine our methods on small-scale webdata as a testbed and then generalize the interventions to a large-scale webgraph containing 93.9M domains and 1.6B edges. We demonstrate that our methods penalize unreliable domains far more than reliable domains in both settings and we explore multiple avenues to mitigate unintended effects on both the small-scale and large-scale webgraph experiments. These results indicate the potential of our approach to reduce the spread of misinformation and foster a more reliable online information ecosystem. This research contributes to the development of targeted strategies to enhance the trustworthiness and quality of search engine results, ultimately benefiting users and the broader digital community.

==> sections/ergm_unused.tex <==

\subsection{ERGM}
Exponential Random Graph Models (ERGMs) attempt to model the stochastic process from which an observed network was generated \cite{robins2007introduction,handcock2008statnet}. ERGMs generate a probability distribution to represent all possible networks and their probabilities of forming ties with the observed network. For a random variable $Y$ representing the state of the network, ERGMs generate the probability of the observed network given network statistics $g(y)$ multiplied by its corresponding network coefficients $\theta$, and normalized by $k(\theta)$, the summation of the numerator's value over all possible networks $y$ with the same nodeset. Formally, this is often written as:

\begin{equation}
P(Y = y\mid \theta) = \frac{exp(\theta^\intercal) g(y)}{k(\theta)}
\end{equation}
This can be re-expressed as the conditional log-odds of a tie between two nodes:
\begin{equation}
    \text{logit}(Y_{ij} = 1\mid y_{ij}^c) = \theta^{\intercal}\delta(y_{ij}) 
\end{equation}
where $\Y_{ij}$ is the random variable for the state of the node pair $i,j$ in the observed network $y_ij$. $y_{ij}^c$ is the complement of the network, and $\delta(y_{ij})$ are the change statistics for each model term. ERGMs allow us to explore the degree to which attributes impact the log-odds an edge forming between $i$ and $j$ conditional on other dyads remaining constant. However, unlike standard logit models, there is no assumption of independence \cite{robins2007introduction}.

We use ERGMs primarily as a tool to better understand the data and explore website reliability influences probability of domains $i$ and $j$ to form a tie. As ERGMs can hold network structures constant, they allow researchers to statistically explore the presence of homophily, transitivity, and other metrics that would violate the assumptions of a standard logit model \cite{williams2020homophily}. We use ERGMs to demonstrate that there is substantial and statistically significant inter-reliability and intra-reliability across domains. Unfortunately, ERGMs struggle to converge on large networks, so we are only able to perform this exploration on a subset of our data \cite{an2016fitting}.

We construct a binary bipartite $m {\times} n$ adjacency matrix $A$ of labeled news domains to backlinking domains. We then calculate the shared backlinking matrix  $A*$ using $A^{\intercal}A$. To reduce noise and make ERGM convergence feasible, we drop edges with a weight of less than 5---in other words we only look at edges reflecting that news domains $i$ and $j$ share at least 5 of the same top backlinking domains. The resulting network is then binarized and all isolates are dropped.

Following the approach of Goodreau \cite{goodreau2007advances}, we first define a null model, then add main effects, and then explore nodal attribute mixing. We evaluate the goodness-of-fit of our models using the Akaike Information Criterion (AIC) and the Bayesian Information Criterion (BIC). While ERGMs violate the \textit{i.i.d.} assumptions of AIC and BIC, a reduction in AIC and BIC has been found to correspond to a better-fit ERGM, consequently AIC and BIC are still widely used to evaluate ERGMs \cite{hunter2008goodness}.




\subsection{ERGM}

To further explore the extent to which targeted intervention is needed, we fit three ERGM models to the shared backlinking-domain network. The network was trimmed so that each remaining edge contains at least 5 shared backlinking domains. We present the results of these models in Table \ref{tbl:ERGM}. Given the large ranges of domain-level backlinks, html pages, and external links, rather using than the most common main effects term, the sum of the sum of attribute $a$ for each $i$ and $j$, we use the sum of the absolute difference between every $i$ and $j$. This allows us to interpret the coefficients as the impact of increasing the absolute difference between $i$ and $j$.

In the Main Effects model and the Node Attribute Mixing model (Attr Mix) we see that increasing the absolute difference in total backlinks between domain $i$ and domain $j$ decreases the log-odds of a tie. In other words, two domains with similar total numbers of backlinks are more likely to share at least 5 top backlinking domains than two domains with very different numbers of total backlinks. The effect is statistically significant at at 0.05 threshhold with (p=0.011) for both models. It seems, therefore, that domains which heavily link to multiple well-known news sites may be less likely to link to more obscure sites. In both models, we observe the opposite effect in the absolute difference of External Links. Sites with highly dissimilar external link counts are more likely to share at least 5 top backlinking domains. This suggests a need to control for the size of websites as we design our regression model and intervention. The absolute difference in HTML pages is not statistically significant.

The main question we want to model with ERGMs concerns how domains are amplified across reliability classes. To capture this effect, we add a node attribute mixture parameter to the model for each possible combination of reliability label (where Unreliable sharing backlinking domains with Unreliable domains is the base). We see the groups combinations most likely to share backlinks are mixed reliability with mixed reliability (log odds of 0.393) and mixed reliability with Reliable domains (0.347). Unreliable domains are also more likely to share links with mixed (0.197) and reliable domains (0.128) than the base case. This backlink crossover further highlights the challenging nature of the problem at hand---naively penalizing sites or links from sites that link to mixed reliability domains would also substantially impact links to reliable domains. Intervention needs to be strategic in order to not unduly penalize reliable domains.

\begin{table}[]
\begin{tabular}{cccc}
& Null Model    & Main Effects   & Attr Mix    \\
Edges & \begin{tabular}[c]{@{}c@{}}-4.479\\ (\textless{}0.01)\end{tabular} & \begin{tabular}[c]{@{}c@{}}-4.495\\ (\textless{}0.01)**\end{tabular}   & \begin{tabular}[c]{@{}c@{}}-4.699\\ (\textless{}0.01)**\end{tabular}    \\
Diff Backlinks                                                               &                                                              &\begin{tabular}[c]{@{}c@{}}-1.06e-10\\ (0.011)*\end{tabular}   & \begin{tabular}[c]{@{}c@{}}-1.08e-10\\ (0.011)*\end{tabular}             \\
Diff HTML pages                                                                &                                                                    & \begin{tabular}[c]{@{}c@{}}1.93e-09\\ (0.766)\end{tabular}             & \begin{tabular}[c]{@{}c@{}}-2.21e-09\\ (0.735)\end{tabular}              \\
Diff Ext. Links                                                                &                                                                    & \begin{tabular}[c]{@{}c@{}}1.54e-09\\ (\textless{}0.01)**\end{tabular} & \begin{tabular}[c]{@{}c@{}}1.74e-09\\ (\textless{}0.01)**\end{tabular} \\
Unreliable-Mixed                                                               &                                                                    &                                                                        & \begin{tabular}[c]{@{}c@{}}0.197\\ (\textless{}0.01)**\end{tabular}     \\
Unreliable-Reliable                                                            &                                                                    &                                                                        & \begin{tabular}[c]{@{}c@{}}0.128\\ (0.039)*\end{tabular}                \\
Mixed-Mixed                                                                    &                                                                    &                                                                        & \begin{tabular}[c]{@{}c@{}}0.393\\ (\textless{}0.01)**\end{tabular}     \\
Mixed-Reliable                                                                 &                                                                    &                                                                        & \begin{tabular}[c]{@{}c@{}}0.347\\ (\textless{}0.01)**\end{tabular}     \\
Reliable-Reliable                                                              &                                                                    &                                                                        & \begin{tabular}[c]{@{}c@{}}0.190\\ (\textless{}0.01)**\end{tabular}     \\ \hline
\begin{tabular}[c]{@{}c@{}}Akaike Information \\      Criterion\end{tabular}   & 55944                                                              & 55910                                                                  & 55865                                                                   \\
\begin{tabular}[c]{@{}c@{}}Bayesian Information \\      Criterion\end{tabular} & 55955                                                              & 55945                                                                  & 55964                                                                  
\end{tabular}
\caption{ERGM model results}
\label{tbl:ERGM}
\end{table}

==> sections/misinfo_sites_section_cut.tex <==
We outline a system of perverse incentives, shielded by an opaque and largely unregulated framework, that allow unreliable news sites to generate profit for their publishers. We argue that parallel to their efforts to defraud ad tech companies and increase reach on social media, publishers of unreliable news sites are incentivized to attempt to game search engine recommendation systems through black-hat Search Engine Optimization (SEO). 

\subsection{Why Misinformation News Websites are Made}

While misinformation and unreliable news sites can be created for partisan or ideological reasons, these sites are often created with a clear profit motive in mind. In their 2019 study, the ad tech experts that Braun and Eklund interviewed claimed that the bulk of hoax news sites they encountered were engaging in a form of \textit{ad fraud} \cite{braun2019fake}. In the most typical case, a publisher sets up a website and employs an inexpensive third party to send `traffic' to their website. This traffic is often some mixture of bot and paid human clicks---examples of what ad tech experts call "invalid traffic" \cite{braun2019fake}. The publisher then tries to monetize their "traffic" by selling ad space to ad tech companies, which in turn administer these ads to the mostly-invalid users. As serving ads to bots does not generate profit, ad tech companies are incentivized to attempt to detect inorganic traffic. Publishers, in response, often attempt to attract organic engagement as this both boosts ad revenue and provides additional camouflage for their mostly-inorganic traffic. 

The desire for organic traffic provides a strong incentive to publish shocking, fake, and sensationalist headlines, as this type of content is an effective way to generate engagement \cite{brady2021social}. Unreliable news stories, particularly political ones, have been found to spread faster than reliable news \cite{vosoughi2018spread}. Numerous news agencies have reported on groups of North Macedonian teenagers who made tens of thousands of dollars off of websites spreading unreliable news about the US 2016 election. One teenager recounts that his most-read articles during the US 2016 election were titled "JUST IN: Obama Illegally Transferred DOJ Money To Clinton Campaign!" and "BREAKING: Obama Confirms Refusal To Leave White House, He Will Stay In Power!" \cite{veles2016}. For publishers, attracting organic traffic with shocking and inflammatory content can translate into advertising revenue.

However, there are other popular "black-hat" ways to gain organic traffic. Websites can use social bots on social media platforms to advertise or simulate engagement. The goal of many of these tactics is to game social media recommendation systems into increasing the visibility of their content. Additionally, website owners can attempt to manipulate search engine traffic by paying for "black-hat" Search Engine Optimization services like link farming. Recent work has revealed that such methods are disproportionately used to promote unreliable news over reliable news \cite{misinformation_detection}.

Ad tech companies typically maintain blocklists of websites or publishers with whom they will not do business, but the effectiveness of blocklists is limited given 1) the huge volume of new websites created each day and 2) the relative ease of evasion \cite{braun2019fake}. Siteefy estimates that in 2023, roughly 250,000 new websites are created each day\footnote{\url{https://siteefy.com/how-many-websites-are-there/}}, so the maintenance of these blocklists would be extremely expensive at best. Further complicating blocklist creation, publishers can engage in evasive tactics like domain spoofing (impersonating another domain) and cloaking (serving one version of a webpage to regular visitors and another version to human or algorithmic moderators) \cite{braun2019fake}. Given this ecosystem benefits purveyors of unreliable news who are incentivized to game search rankings, algorithmic approaches are needed to counter attempted manipulations.


